Print-N-Grip: A Disposable, Compliant, Scalable and One-Shot 3D-Printed Multi-Fingered Robotic Hand

Robotic hands are an important tool for replacing humans in handling toxic or radioactive materials. However, these are usually highly expensive, and in many cases, once they are contaminated, they cannot be re-used. Some solutions cope with this challenge by 3D printing parts of a tendon-based hand. However, fabrication requires additional assembly steps. Therefore, a novice user may have difficulties fabricating a hand upon contamination of the previous one. We propose the Print-N-Grip (PNG) hand which is a tendon-based underactuated mechanism able to adapt to the shape of objects. The hand is fabricated through one-shot 3D printing with no additional engineering effort, and can accommodate a number of fingers as desired by the practitioner. Due to its low cost, the PNG hand can easily be detached from a universal base for disposing upon contamination, and replaced by a newly printed one. In addition, the PNG hand is scalable such that one can effortlessly resize the computerized model and print. We present the design of the PNG hand along with experiments to show the capabilities and high durability of the hand.

==> method.tex <==
\section{Analytical Model}

% Assumptions
We assume that the joints are stiff enough such that effects of gravity can be neglected. Furthermore, finger motions are considered quasi-static such that dynamic effects are neglected.


Kinematic analysis of an underactuated hand \cite{Wang2011}.


\begin{equation}
    J^{T}\ve{f}=T^{-T}\ve{\tau}
\end{equation}
where $J$ is the Jacobian of the finger, $\ve{f}$ is the vector of forces on the links, $T$ is the transmission matrix and $\tau$ is the vector of joint torques. Check in \cite{Birglen2008}???
